AU Microscopii in the FUV: Observations in Quiescence, During Flares, and Implications for AU Mic b and c

High energy X-ray and ultraviolet (UV) radiation from young stars impacts planetary atmospheric chemistry and mass loss. The active $\sim 22$ Myr M dwarf AU Mic hosts two exoplanets orbiting interior to its debris disk. Therefore, this system provides a unique opportunity to quantify the effects of stellar XUV irradiation on planetary atmospheres as a function of both age and orbital separation. In this paper we present over 5 hours of Far-UV (FUV) observations of AU Mic taken with the Cosmic Origins Spectrograph (COS; 1070-1360 Angstrom) on the Hubble Space Telescope (HST). We provide an itemization of $120$ emission features in the HST/COS FUV spectrum and quantify the flux contributions from formation temperatures ranging from $10^4-10^7$ K. We detect 13flares in the FUV white-light curve with energies ranging from $10^{29} - 10^{31}$ ergs. The majority of the energy in each of these flares is released from the transition region between the chromosphere and the corona. There is a 100$\times$ increase in flux at continuum wavelengths $\lambda < 1100$ Angstrom in each flare which may be caused by thermal Bremsstrahlung emission. We calculate that the baseline atmospheric mass-loss rate for AU Mic b is $\sim 10^8$ g s$^{-1}$, although this rate can be as high as $\sim 10^{14}$ g s$^{-1}$ during flares with $L_\textrm{flare} \simeq 10^{33}$ erg s$^{-1}$. Finally, we model the transmission spectra for AU Mic b and c with a new panchromatic spectrum of AU Mic c and motivate future JWST observations of these planets.

==> style.tex <==
% Packages
\usepackage{xifthen}
\usepackage{stackengine}
\usepackage{tabstackengine}
\usepackage{array}
\usepackage{upgreek}
\usepackage[bbgreekl]{mathbbol}
\usepackage{afterpage}
\usepackage[bb=boondox]{mathalpha}

% Shorthand for this paper
\newcommand{\starry}{\textsf{starry}\xspace}
\newcommand{\celerite}{\textsf{celerite}\xspace}
\newcommand{\cpp}{\textsf{C++}\xspace}
\newcommand{\theano}{\textsf{theano}\xspace}
\newcommand{\pymcthree}{\textsf{pymc3}\xspace}
\newcommand{\starryprocess}{\textsf{starry\_process}\xspace}
\newcommand{\Python}{\textsf{Python}\xspace}
\newcommand{\xxx}[1]{{\color{red}#1}}
\newcommand{\quadquad}{\quad\quad\quad\quad}

% Misc. macros
\newcommand{\LMAX}{15\xspace}

% Integrals
\newcommand{\dd}{\ensuremath{\text{d}}}

% Special functions
\newcommand{\sgn}{{\text{sgn}}}
\newcommand{\atantwo}{{\text{arctan2}}}

% Cartesian unit vectors
\newcommand{\xhat}{\ensuremath{\pmb{\hat{x}}}\xspace}
\newcommand{\yhat}{\ensuremath{\pmb{\hat{y}}}\xspace}
\newcommand{\zhat}{\ensuremath{\pmb{\hat{z}}}\xspace}

% Other
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% Inverse diagonal dots
\makeatletter
\def\Ddots{\mathinner{\mkern1mu\raise\p@
                \vbox{\kern7\p@\hbox{.}}\mkern2mu
                \raise4\p@\hbox{.}\mkern2mu\raise7\p@\hbox{.}\mkern1mu}}
\makeatother

% Imaginary unit
\DeclareFontFamily{U}{mathc}{}
\DeclareFontShape{U}{mathc}{m}{it}{<->s*[1.03] mathc10}{}
\DeclareMathAlphabet{\mathscr}{U}{mathc}{m}{it}
\DeclareMathOperator{\imag}{\mathscr{i}}

